Resilient Cloud Control System: Realizing resilient cloud-based optimal control for cyber-physical systems

The transformation to smart factories and the automation of mobile robotics is partly driven by a growing availability of ubiquitous cloud technologies. In cyber-physical systems, such as control systems, critical parts can be migrated to a cloud for offloading, enabling collaborative processes, improved performance, and life-cycle management. Despite the performance uncertainty in a cloud and the intermediate networks, presently, even cloud native function services are being investigated for supporting critical applications that are sensitive to time-varying execution and communication delays. In this paper, we introduce, implement, and empirically evaluate an architecture that successfully allows predictive controllers to take advantage of cloud native technology. Our solution relies on continuously adapting the control system to the present Quality of Service of the cloud and the intermediate network. As our results show, this allows a control system to survive interruptions, noisy neighbors, and time-variant resource availability. Without the proposed solution, the control system will fail due to resource constraints and insufficient response times. Further, we also show a system that can seamlessly switch between clouds and that multiple controllers using shared resources consequentially self-adapt so that no controller fails its objective.

==> sections/discussion.tex <==
\section{Discussion}
[I suggest we try the IMRaD format to create credibility. Since we have many sections in the results we can extract the discussion and likely shorten and focus the text]

==> sections/introduction_alternative.tex <==
Automation has never been as abundant as it is today.
\textit{Intelligent} systems are entering our everyday lives in various forms, while the Fourth Industrial Revolution (Industry 4.0) promises competitive advantages to companies that take a leap in automation technology.
It is forecast that already in in 2022, 18 billion \ac{IoT} devices will be connected to the Internet.

In this era, feedback controller are outgrowing their traditional production platforms and are bound for a cloud where they can be offloaded, collaborate, and scale to the desired size.
While of-the-shelf cloud and \ac{IoT} technology is reaching a level of maturity that is ripe for factory automation~\cite{khan2017analysis,8473376,skarin2020cloudperformance}, closed loop control systems have yet to make its big entry on these platforms.
Nevertheless, the cloud is an noise environment for mission-critical and time-sensitive processes, such as feedback controllers. 
Time-variant execution and communication delay and jitters is innate to cloud deployments and can be catastrophic to the controller and the process under control.
While \ac{IIoT} and the underpinning cloud platforms and wireless networks are evolving and maturing, it is still challenging to ensure desired real-time properties~\cite{9134804} for resident applications.
Arguably, some degree of uncertainty is inherit and is unavoidable.
Nevertheless, incorporating clouds into production platforms allows for new types of control applications to emerge when up front costs are translated into pay-as-you-go, when processes share data, and when processes collaborate. 

Conventional wisdom from \ac{NCS} does not address the challenges imposed on controllers by the cloud.
There are several works on control over shared networks that consider on-line adaptation for sharing and resource preservation, for instance~\cite{ploplys2004closed,xia2007flexible}.
Applied to controllers deployed in the cloud, the literature has the following shortcomings:
\begin{inparaenum} 
    \item assuming a single distribution of delays,
    \item assuming limited range in the variability of delays, i.e., no fat tails or complete disconnects,
    \item considering only the network as a source of error, and
    \item a focus on simple controllers that are not intrinsically useful in the cloud context~\cite{7ad724ad6a2c47368b0507e57cadb1bc}, for instance PIDs.
\end{inparaenum}
In addition, many results rely on conservative systems that must assume the worst in order to provide stability and performance guarantees, something that is simply not applicable when we allow the control system to arbitrarily disconnect.

In this paper, we introduce \ac{R-CCS}. A set of design principals for predictive controllers to successfully and continuously run and take advantage of any cloud.
Our solution fundamentally relied on adapting the controller to prevailing conditions in the cloud.
As our results show, the this allows the system to survive interruptions, noisy neighbors, and time-varying resource availability.
Without our solutions, the processes fail. 
Further, our experiments also show that the system can seamlessly switch between clouds and that multiple controllers using the same cloud resources self-adapt so that no controller is starved.

==> sections/targeted-system.tex <==

    % \subsection{Switched systems} %\reviewwilliam{Again, this is out of scope at this point, we have not presented enough detail about the system to warrant switching. A reader/reviwer will probably not understand how this is relevant. Otherwise, well written.}
    % 	Switched systems exhibit modes in which the system dynamics change.
    % 	Changes can be due to external events, such as a group policy in a population, or selectively, such as in a piece-wise linear approximation of a non-linear system.
    % 	For instance, in a radio transmitter the transmission model and control strategy may change with frequency and output gain.
    % 	Switching can in itself cause degraded performance and system instability.
    % 	This is true even if every individual mode is capable of controlling the system in isolation.
    % 	Switching control theory deals with bounding the rate of changes and finding efficiently controllers that work reliably with more or less arbitrary switching between plant models and control strategies.
    
     %what makes them performant.% and the distinguishing features we identify with the cloud.

%     \subsection{Feedback control} \reviewwilliam{Have we established in the introduction the notion of a feedback control system?}
%         In feedback control, a dynamic system referred to as the \emph{\plantorprocess{}} is manipulated by a
%         %A \plantorprocess{} can be an isolated system such as the joint of a robotic arm, or a large and complex combination of hundreds of valves and switches in a production plant.
%         \emph{controller}.
%         The controller is another dynamic system purposefully created to achieve a set of performance \emph{objectives}, such as moving a robotic arm to a new position within a certain time and with a limited degree of error.
%         To capture such behaviors and dynamics, a controller often relies on a \emph{model} that represents the physical system and possibly its environment.
%         %Model simplifications, parameter estimations, measurement errors, and unknown disturbances from the environment, incur additional complexity in controlling the plant.
%         The basic problem is in deriving a controller that can manipulate the targeted \plantorprocess{} to meet the system's objectives and performance goals.
% 		Model abstractions, parameter estimations, execution platform requirements and system disturbances incur additional complexities that are addressed with tools from the field of feedback control.
% 		\reviewwilliam{A reference to MPC $>>>$ ML?}
% 		%In extension, it also involves finding a representative model, tuning model parameters, formalizing objectives and performance goals, and handling disturbances in the environment.

%     \subsection{Computer controlled systems}
%         Feedback control systems are mostly realized as discrete-time, often periodic, applications with strict timing requirements.
% 		Unless the hosting platform's performance follows strict rules, it may be challenging, or impossible, to meet a control system's requirements.
%         Consequently, feedback controllers are conventionally implemented on industrial grade hardware that have close to deterministic execution times and long mean time between failures, such as proprietary \acp{PLC}.
%         A great deal of care is taken to ensure that controllers execute timely, periodically, and that synchronization of signaling, i.e. sensory input and control output, is well understood.
%         \reviewwilliam{Should these last two sentences be put in section below about optimal controllers?}
% 		Real-time predictive controllers, such as the \ac{MPC} in this paper, rely on optimization frameworks with extensive and variable execution times. It is not uncommon to implement them on general purpose hardware and software platforms,
% 		paving the way for the transition to cloud deployed \acp{MPC}.
        

% 	\subsection{Optimal control and constrained systems}
%     	Optimal control uses plant, disturbance and system models (such as delays) in combination with a \textit{cost function} to find an optimal feedback control strategy. \reviewwilliam{Plant or process? I think process is more in line with expectations at IC2E.}
%     	In theoretical, unconstrained and linear systems, efficient strategies can be implemented through predetermined analytical solutions.
%     	Switching (see the following section) and large safety margins can be used to create conditions in which these properties can be assumed.
%     	An alternative is to solve the control problem on-line, leading again to the \ac{MPC}.
%     	This is convenient from an engineering perspective, allowing the insertion of constraints and non-linear models into the on-line optimization.
%     	The downside is that this requires a lot more computations in real-time and that the execution time of the controller can vary.
%     	On-line optimization is an attractive choice for use with the cloud because the computational requirements are traded in for great convenience and control performance.

%		The studied \ac{CCS} implements \ac{MPC} which is an explicit, online, optimizing control strategy.

%     \subsection{Networked control} \label{sec:network_control} \reviewwilliam{At this point we have not established what \ac{CCS} is, nor that the controller is separated from the process over a network. Therefore this will make little sense to a reviewer.}
%         The typical notion of \emph{networked control} implies that the sensory data, the input to the controller, or actuator inputs, the control signals, are transferred over a network. 
%         This introduces stochastic network delay and packet loss into the closed loop system.
%         %Networked critical control is depicted in \Cref{fig:basicnetcontrol}.
%         %Here, networked control is critical because the control must function over an unreliable network or the plant objective will fail.
%         Network control theory studies the requirements that must apply to the communication channel in order for the overall system to meet the objectives and not malfunction.
%         An example is found in \cite{kim2005network}, which studies the control of a Maglev system over the Internet.
%         This work experimentally verifies that the closed loop requires no more than three successive packet losses in order to remain functional.
%         This is a strict requirement that the execution platform must fulfill since the controller is directly manipulating the plant.

%         Another type of networked control is shown in \Cref{fig:supervisorycontrol}. \reviewwilliam{May be too early for \Cref{fig:cloud-control-solution}?}
%         Here, the plant is not directly manipulated over the network.
% 		An independent, local control loop is acting on the \plantorprocess{} to fulfill some current objectives, as defined by a \emph{supervisor controller}.
%         The supervisor sets the parameters of the local controller but is not responsible for generating the final input signal to the plant.
% 		Supervisory control is also present in \cite{kim2005network}, in terms of of manual configuration of the Maglev controller through a web page.
% 		In more advanced setups, network control theory can be used to study the performance of the combined system, and ensure that frequent configuration changes do not cause issues.
% 		In general, the problem consists in finding the bounds on uncertainty of a system, and designing a cost effective platform thereafter, or finding the best performing controller (the least conservative) given the bounded uncertainty of a platform.
    

==> tables/target_rtt.tex <==
\begin{tabular}{cllll}
\toprule
Index & Target       & Median & \nth{75} quantile & \nth{95} quantile \\ 
\midrule
0 & bbk8s        & 11.71 ms               & 12.35 ms                          & 12.82 ms                           \\ 
1 & erdc         & 24.24 ms               & 25.34 ms                          & 26.46 ms                          \\ 
2 & eu-central-1 & 37.55 ms               & 39.97 ms                         & 52.62 ms                          \\ 
3 & eu-north-1   & 180.06 ms              & 199.06 ms                        & 218.57 ms                       \\
\bottomrule
\end{tabular}


==> texfigures/tikzctrllib.tex <==
\tikzset{
	plant/.style = {rounded corners, thick},
	sharp/.style = {sharp corners},
	smooth/.style = {rounded corners},
	redshade/.style = {draw=red, left color=red!20!white, right color=red!70!white},
	blueshade/.style = {draw=blue, left color=blue!20!white, right color=blue!70!white},
	greenshade/.style = {draw=green, left color=green!20!white, right color=green!70!white},
	yellowshade/.style = {draw=yellow, left color=yellow!20!white, right color=yellow!70!white},
	grayshade/.style = {black,draw=black, left color=black!20!white, right color=black!50!white},
	blackshade/.style = {white, draw=black, left color=black!60!white, right color=black!90!white},
	whiteshade/.style = {black, draw=white!60!black, left color=white, right color=white!60!black},
}

